Impact of COVID-19 on Public Transit Accessibility and Ridership

Public transit is central to cultivating equitable communities. Meanwhile, the novel coronavirus disease COVID-19 and associated social restrictions has radically transformed ridership behavior in urban areas. Perhaps the most concerning aspect of the COVID-19 pandemic is that low-income and historically marginalized groups are not only the most susceptible to economic shifts but are also most reliant on public transportation. As revenue decreases, transit agencies are tasked with providing adequate public transportation services in an increasingly hostile economic environment. Transit agencies therefore have two primary concerns. First, how has COVID-19 impacted ridership and what is the new post-COVID normal? Second, how has ridership varied spatio-temporally and between socio-economic groups? In this work we provide a data-driven analysis of COVID-19's affect on public transit operations and identify temporal variation in ridership change. We then combine spatial distributions of ridership decline with local economic data to identify variation between socio-economic groups. We find that in Nashville and Chattanooga, TN, fixed-line bus ridership dropped by 66.9% and 65.1% from 2019 baselines before stabilizing at 48.4% and 42.8% declines respectively. The largest declines were during morning and evening commute time. Additionally, there was a significant difference in ridership decline between the highest-income areas and lowest-income areas (77% vs 58%) in Nashville.

==> figures/void/ChattanoogaBaseline.tex <==
\begin{figure}[t]
    \centering
%\pgfplotsset{scaled y ticks=false}
\begin{tikzpicture}
\begin{axis}[
    width=.8\columnwidth,
    height=.5\columnwidth,
    font=\footnotesize,
    % yaxis
    %ymin = -100, ymax = 100,
    ytick={-80, -60, -40, -20, 0, 20, 40},
    yticklabel style={anchor=near yticklabel},
    yticklabel={$\pgfmathprintnumber{\tick}\%$},
    ylabel={Change in Ridership},
    % xaxis
    xlabel=Month,
    date coordinates in=x,
    xtick={ % ticks at first day of each month
    2020-2-1,
    2020-3-1,
    2020-4-1,
    2020-5-1,
    2020-6-1},
    xticklabel style={rotate=45,anchor=near xticklabel},
    xticklabel={\pgfcalendarmonthshortname{\month}},
    date ZERO=2009-08-18,% <- improves precision!
	enlarge x limits=false,
    ]
    \addplot+[blue, mark=none, fill=blue!10!white] table [col sep=comma, x=date, y=change]
    {data/ChattanoogaBaseline.csv} \closedcycle;
    \addplot+[black, mark=none] coordinates {(2020-2-9, 0) (2020-6-28, 0)};
\end{axis}
\end{tikzpicture}
    \caption{Weekly change in ridership for Chattanooga, TN.}
    \label{fig:ChattanoogaBaseline}
    \vspace{-0.8em}
\end{figure}

==> figures/void/NashvilleBaseline.tex <==
\begin{figure}[t]
    \centering
%\pgfplotsset{scaled y ticks=false}
\begin{tikzpicture}
\begin{axis}[
    width=.8\columnwidth,
    height=.5\columnwidth,
    font=\footnotesize,
    % yaxis
    %ymin = -100, ymax = 100,
    ytick={-80, -60, -40, -20, 0, 20, 40},
    yticklabel style={anchor=near yticklabel},
    yticklabel={$\pgfmathprintnumber{\tick}\%$},
    ylabel={Change in Ridership},
    % xaxis
    xlabel=Month,
    date coordinates in=x,
    xtick={ % ticks at first day of each month
    2020-2-1,
    2020-3-1,
    2020-4-1,
    2020-5-1,
    2020-6-1},
    xticklabel style={rotate=45,anchor=near xticklabel},
    xticklabel={\pgfcalendarmonthshortname{\month}},
    date ZERO=2009-08-18,% <- improves precision!
	enlarge x limits=false,
    ]
    \addplot+[blue, mark=none, fill=blue!10!white] table [col sep=comma, x=date, y=change]
    {data/NashvilleBaseline.csv} \closedcycle;
    \addplot+[black, mark=none] coordinates {(2020-2-9, 0) (2020-6-28, 0)};
\end{axis}
\end{tikzpicture}
    \caption{Weekly change in ridership for Nashville, TN.}
    \label{fig:NashvilleBaseline}
    \vspace{-0.8em}
\end{figure}

==> figurescombined/RidershipChangeAccidents.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{.5\linewidth}
        \input{figures/Baseline}
        \caption{Nashville}
        \label{subfig:BoardingCovidcases1}
    \end{subfigure}%
    \begin{subfigure}[t]{.5\linewidth}
        \input{figures/NashvilleAccidents}
        \caption{Chattanooga}
        \label{subfig:BoardingCovidcases2}
    \end{subfigure}
    \caption{TODO}
    \label{fig:RidershipChangeAccidents}
\end{figure}

==> figurescombined/Socio.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{.8\linewidth}
        \input{figures/NashvilleCensusLinePlot}
        \caption{}
        \label{subfig:t}
    \end{subfigure}%
    \begin{subfigure}[t]{.2\linewidth}
        \input{figures/NashvilleCorrelation}
        \caption{}
        \label{subfig:j}
    \end{subfigure}
    \caption{TODO}
    \label{fig:Socio}
\end{figure}
